Worse WER, but Better BLEU? Leveraging Word Embedding as Intermediate in Multitask End-to-End Speech Translation

Speech translation (ST) aims to learn transformations from speech in the source language to the text in the target language. Previous works show that multitask learning improves the ST performance, in which the recognition decoder generates the text of the source language, and the translation decoder obtains the final translations based on the output of the recognition decoder. Because whether the output of the recognition decoder has the correct semantics is more critical than its accuracy, we propose to improve the multitask ST model by utilizing word embedding as the intermediate.

==> sections/sect4.tex <==

\section{Experimental Setup}
\label{expsetup}
\subsection{Data}
\label{data}
We used Fisher Spanish corpus~\cite{fishercorpus} to perform Spanish speech to English text translation. 
And we followed previous works~\cite{inaguma2019multilingual} for pre-processing steps, and 40/160 hours of \emph{train} set, standard \emph{dev}-\emph{test} are used for the experiments.
Byte-pair-encoding (BPE)~\cite{kudo2018sentencepiece} was applied to the target transcriptions to form 10K subwords as the target of the translation part.
Spanish word embeddings were pre-trained on Wikipedia, which can be obtained from FastText~\cite{bojanowski2016enriching}, and 8000 Spanish words were used in the recognition part.



\subsection{Implementation}
\label{implementation}
Encoder is a 3-layer 512-dimensional bidirectional LSTM with additional convolution layers, yielding 8$\times$ down-sampling in time.
Decoders are 1024-dimensional LSTM, and we used one layer in the recognition part and two layers in the translation part.
Models were optimized using Adadelta with $10^{-6}$ as the weight decay rate.
Scheduled sampling with probability 0.8 was applied on the target language decoder.
Experiments ran 1.5M steps, and models were selected by the highest BLEU on four references per speech on \emph{dev} set.
